Segment Anything Model for Grain Characterization in Hard Drive Design

Development of new materials in hard drive designs requires characterization of nanoscale materials through grain segmentation. The high-throughput quickly changing research environment makes zero-shot generalization an incredibly desirable feature. For this reason, we explore the application of Meta's Segment Anything Model (SAM) to this problem. We first analyze the out-of-the-box use of SAM. Then we discuss opportunities and strategies for improvement under the assumption of minimal labeled data availability. Out-of-the-box SAM shows promising accuracy at property distribution extraction. We are able to identify four potential areas for improvement and show preliminary gains in two of the four areas.

==> sec/results.tex <==
\section{Results}
\label{sec:results}
Text

Individual Grains Comparison. Prompt selection, thresholding, multimask output.


Comparison of SAM Full Image mask generator to new. In terms of time and accuracy.


